Don't Start from Scratch: Behavioral Refinement via Interpolant-based Policy Diffusion

Imitation learning empowers artificial agents to mimic behavior by learning from demonstrations. Recently, diffusion models, which have the ability to model high-dimensional and multimodal distributions, have shown impressive performance on imitation learning tasks. These models learn to shape a policy by diffusing actions (or states) from standard Gaussian noise. However, the target policy to be learned is often significantly different from Gaussian and this mismatch can result in poor performance when using a small number of diffusion steps (to improve inference speed) and under limited data. The key idea in this work is that initiating from a more informative source than Gaussian enables diffusion methods to mitigate the above limitations. We contribute both theoretical results, a new method, and empirical findings that show the benefits of using an informative source policy. Our method, which we call BRIDGER, leverages the stochastic interpolants framework to bridge arbitrary policies, thus enabling a flexible approach towards imitation learning. It generalizes prior work in that standard Gaussians can still be applied, but other source policies can be used if available. In experiments on challenging simulation benchmarks and on real robots, BRIDGER outperforms state-of-the-art diffusion policies. We provide further analysis on design considerations when applying BRIDGER. Code for BRIDGER is available at https://github.com/clear-nus/bridger.

==> sections/cost_improvement.tex <==
\begin{assumption}[Optimal Density]
    Let $c$ be a cost function. The optimal density
    \begin{equation*}
        p^*(x)=\frac{1}{Z}\exp(-c(x))
    \end{equation*}
    where $Z$ is a normalizing constant.
\end{assumption}

\begin{assumption}[Bounded Improvement]
    There exist constants $\epsmax>\epsmin>0$ such that for all $t\in[T]$,
    \begin{equation*}
        H(p_{t-1},p^*)-\epsmax\leq H(p_t,p^*)\leq H(p_{t-1},p^*)-\epsmin.
    \end{equation*}
    We can interpret $\epsmin$ and $\epsmax$ as the minimum and maximum improvement after each diffusion step.
\end{assumption}

\begin{lemma}
    Let $t\in\{1,\dots,T\}$. Then $\E_{x\sim p_t}[c(x)]\leq\E_{x\sim p_{t-1}}[c(x)]-\epsmin$.
\end{lemma}

\begin{proof}
    We bound the expectation directly.
    \begin{align*}
        \E_{x\sim p_t}[c(x)]
        &=\int p_t(x)c(x)\,dx\\
        &=-\int p_t(x)\ln(Zp^*(x))\,dx\\
        &=-\int p_t(x)\ln(Z)\,dx-\int p_t(x)\ln(p^*(x))\,dx\\
        &=-\ln(Z)+H(p_t,p^*)\\
        &\leq-\ln(Z)+H(p_{t-1},p^*)-\epsmin\\
        &=-\int p_{t-1}(x)\ln(Z)\,dx-\int p_{t-1}(x)\ln(p^*(x))\,dx-\epsmin\\
        &=-\int p_{t-1}(x)\ln(Zp^*(x))\,dx-\epsmin\\
        &=\int p_{t-1}(x)c(x)\,dx-\epsmin\\
        &=\E_{x\sim p_{t-1}}[c(x)]-\epsmin.\qedhere
    \end{align*}
\end{proof}

\clearpage

\begin{lemma}
    Let $t\in\{1,\dots,T\}$. Then $\E_{x\sim p_t}[c(x)]\geq\E_{x\sim p_{t-1}}[c(x)]-\epsmax$.
\end{lemma}

\begin{proof}
    We bound the expectation directly.
    \begin{align*}
        \E_{x\sim p_{t-1}}[c(x)]
        &=\int p_{t-1}(x)c(x)\,dx\\
        &=-\int p_{t-1}(x)\ln(Zp^*(x))\,dx\\
        &=-\int p_{t-1}(x)\ln(Z)\,dx-\int p_{t-1}(x)\ln(p^*(x))\,dx\\
        &=-\ln(Z)+H(p_{t-1},p^*)\\
        &\leq-\ln(Z)+H(p_{t},p^*)+\epsmax\\
        &=-\int p_t(x)\ln(Z)\,dx-\int p_t(x)\ln(p^*(x))\,dx+\epsmax\\
        &=-\int p_t(x)\ln(Zp^*(x))\,dx+\epsmax\\
        &=\int p_t(x)c(x)\,dx+\epsmax\\
        &=\E_{x\sim p_t}[c(x)]+\epsmax.\qedhere
    \end{align*}
\end{proof}

\begin{theorem}
    Let $p_0$ and $p_0'$ be priors such that $\E_{x\sim p_0}[c(x)]\leq\E_{x\sim p_0'}[c(x)]$. Then we have
    \begin{equation*}
        \E_{x\sim p_T}[c(x)]\leq\E_{x\sim p_T'}[c(x)]+T(\epsmax-\epsmin).
    \end{equation*}
\end{theorem}

\begin{proof}
    We prove by induction. When $t=1$, we have
    \begin{align*}
        \E_{x\sim p_1}[c(x)]-\E_{x\sim p_1'}[c(x)]
        &\leq (\E_{x\sim p_0}[c(x)]-\epsmin)-(\E_{x\sim p_0'}[c(x)]-\epsmax)\\
        &= \E_{x\sim p_0}[c(x)]-\E_{x\sim p_0'}[c(x)]+(\epsmax-\epsmin)\\
        &\leq \epsmax-\epsmin.
    \end{align*}
    Now assume $\E_{x\sim p_t}[c(x)]\leq\E_{x\sim p_t'}[c(x)]+t(\epsmax-\epsmin)$. Then
    \begin{align*}
        \E_{x\sim p_{t+1}}[c(x)]-\E_{x\sim p_{t+1}'}[c(x)]
        &\leq (\E_{x\sim p_t}[c(x)]-\epsmin)-(\E_{x\sim p_t'}[c(x)]-\epsmax)\\
        &= \E_{x\sim p_t}[c(x)]-\E_{x\sim p_t'}[c(x)]+(\epsmax-\epsmin)\\
        &\leq t(\epsmax-\epsmin)+(\epsmax-\epsmin)\\
        &\leq (t+1)(\epsmax-\epsmin).\qedhere
    \end{align*}
\end{proof}

==> sections/rebuttal.tex <==
\section*{General Response}

We thank the area chair (\ac{}) and reviewers (\rone{} [4wGh], \rtwo{} [v8bq], \rthree{} [9Mic]) for your positive comments about novelty and rigor, and  your constructive feedback. We have incorporated your comments into our revision. Edits to the manuscript are shown in \rev{blue}. 

\para{Real robot experiments (\ac{}, \rtwo{}, \rthree{}).} The main concern raised was about the lack of real-world robot experiments. To address this concern, our paper now includes an entirely new section (Sec \ref{sec:rw_experiment}) on two real robot  experiments: 
\begin{itemize}
    \item Stable grasping using a Franka Emika Panda arm with a two-finger Robotiq 2F-140 gripper;
    \item Synthetic wound cleaning using a UR5e equipped with a Shadow Dexterous Hand Lite.
\end{itemize} 
These tasks involved real high-dimensional observations (e.g., point clouds and images) and complex actions. To our knowledge, the cleaning task has the \emph{highest} action sequence dimension ($22\times48$ to control the arm and Shadow hand) among reported real robot tasks using diffusion models. Further, it involves manipulation of a soft deformable sponge to perform the cleaning task.  

Results show that \emph{our method achieves better performance compared to state-of-the-art diffusion methods for imitation learning}. 
Please also see the new video ({\small\texttt{bridger\_video\_realworld.mp4}}) in the supplementary material that shows the differences when applying \method{} compared to diffusion policies --- \method{}'s trajectories are smoother and more accurate, especially when performing 5 diffusion steps for faster inference. We believe that these results makes clear the significance of our work for robotics. 

\para{Writing quality (\ac{}, \rone{}, \rtwo{}).} We have edited the paper to improve clarity, given the technical nature of the method. A specific concern raised was that jargon was used before explanation (\rtwo{}) and we have adopted \rtwo{}'s suggestion to include short explanations in the introduction. Proofs are in the appendix. We have also added clarifying remarks to address specific comments/questions raised by the reviewers. 

\section*{Specific Responses to \rone{} [4wGh]}

\para{Training loss in Algorithm 2 might be prone to convergence on local minima.} We do not clearly understand this comment so please forgive any misunderstanding. The training loss is similar to diffusion models (a L2 loss), except that we learn the velocity and its decomposed form. Local minima are generally unavoidable when using nonlinear functions (e.g., deep neural networks) to parameterize the learnt functions; this applies to diffusion policies as well. However, in practice, diffusion methods (incl. \method{}) are able to learn good policies.   

\para{Supplementary video does not clearly demonstrate the superiority of the proposed method.} We have added new videos on the real world robots that show differences more clearly. Please note that the earlier videos were intentionally designed to show both success and failure cases (across methods) for completeness.  

\begin{figure}
\begin{center}
   \includegraphics[width=0.8\linewidth]{figures/real_robot/real-robot-tasks-reb.pdf} 
   \caption*{Real Robot Experiments in Section \ref{sec:rw_experiment}.}
\end{center}
\vspace{-1.5em}
\end{figure}

\section*{Specific Responses to \rtwo{} [v8bq]}
We hope that the addition of real-world robot experiments (Sec. \ref{sec:rw_experiment}) makes clear the relevance of our work to robotics. 

\para{BRIDGeR sometimes degrades in performance with more diffusion steps.} This sometimes occurs for \method{} and also for DDIM . We posit that this is due to the accumulation of numerical/prediction errors during the forward simulation of the SDE. We mention this in Sec \ref{sec:rw_experiment} of the revision, but leave a more thorough investigation to future work. 

\para{Report the success rates of the CVAE source policy as a baseline.} Indeed, we agree this is important and reported the success rates of the source policies as \method{} with $k=0$ in our tables and as the ``Source'' in Figure 10. We have edited the caption in Table I and Figure 10 to clarify this. 

\para{Performance of the Residual Policy and implementation.} We specified the Residual Policy setup in Appendix D. Its performance is low because it is a regression model that doesn't capture multimodal distributions. Specifically, it is trained to predict the difference between a source action and target action. During test time, the predicted difference is added to an action sampled from the source distribution. We will release source code which provides implementation details.

\section*{Specific Responses to \rthree{} [9Mic]}
We hope that the results from real-world robot experiments (Sec. \ref{sec:rw_experiment}) using real RGB image and point cloud observations makes clear the relevance and practicality of our work. 

\para{Meaning of reported performance numbers for Adriot tasks.} The reported numbers are success rates (a trial is successful if the cumulative reward exceeds a threshold). We have edited Appendix B to specify how the success rates were determined and will release source code to reproduce these metrics and our experiments. 

\section*{Summary to AC and All Reviewers}
Thank you again for your valuable comments. We hope our real-world experiments and edits to the paper have  clarified our approach along with its significance for robotics. If we have addressed your concerns, we hope you will consider revising your recommendation towards acceptance. 

\newpage
